Inference for BART with Multinomial Outcomes

The multinomial probit Bayesian additive regression trees (MPBART) framework was proposed by Kindo et al. (KD), approximating the latent utilities in the multinomial probit (MNP) model with BART (Chipman et al. 2010). Compared to multinomial logistic models, MNP does not assume independent alternatives and the correlation structure among alternatives can be specified through multivariate Gaussian distributed latent utilities. We introduce two new algorithms for fitting the MPBART and show that the theoretical mixing rates of our proposals are equal or superior to the existing algorithm in KD. Through simulations, we explore the robustness of the methods to the choice of reference level, imbalance in outcome frequencies, and the specifications of prior hyperparameters for the utility error term. The work is motivated by the application of generating posterior predictive distributions for mortality and engagement in care among HIV-positive patients based on electronic health records (EHRs) from the Academic Model Providing Access to Healthcare (AMPATH) in Kenya. In both the application and simulations, we observe better performance using our proposals as compared to KD in terms of MCMC convergence rate and posterior predictive accuracy.

==> commands.tex <==
\section{Common commands}
\label{sec:commoncmds}

The \MP{} manual~\cite{hobby:user} lists 26 built-in commands along with
23 function-like macros for which pictures can be drawn and manipulated
using \MP.  We will not discuss each of these commands here; however, we
will focus on several of the most common commands and provide examples
of their usage.

\input{draw}
\input{fill}
\input{arrows}
\input{label}

